Soft Weight-Sharing for Neural Network Compression

The success of deep learning in numerous application domains created the de- sire to run and train them on mobile devices. This however, conflicts with their computationally, memory and energy intense nature, leading to a growing interest in compression. Recent work by Han et al. (2015a) propose a pipeline that involves retraining, pruning and quantization of neural network weights, obtaining state-of-the-art compression rates. In this paper, we show that competitive compression rates can be achieved by using a version of soft weight-sharing (Nowlan & Hinton, 1992). Our method achieves both quantization and pruning in one simple (re-)training procedure. This point of view also exposes the relation between compression and the minimum description length (MDL) principle.

==> tables/exp1_init.tex <==
\begin{table}[hbt!]
%\caption{INIT BLABLABAL LeNet-300-100}
\label{sample-table}
\begin{center}
\begin{tabular}{lcccccc}
\hline 
Method &  Error [\%] & Comp. rate & Non-zeros [\%]&$\max(\sigma_j^2)$ & $\text{mean}(\sigma_j^2)$ &$\text{Var}(\sigma_j^2)$\\ 
\hline  \hline 
Reference			&1.89  & - & - & - & - & -\\	
Initial Run  		&1.94  & 62.2  & 0.04 &  $1.045 $&$ 0.142 $&$ 0.090 $\\
\hline
\end{tabular}
\end{center}
\label{table:init}
\end{table}

==> tables/exp1_t1.tex <==
\begin{table}[hbt!]
%\caption{INIT BLABLABAL LeNet-300-100}
\label{sample-table}
\begin{center}
\begin{tabular}{lccccccc}
\hline 
$(\lambda^*)^{-1}$& $\text{var}_\gamma$ &  Error [\%] & Comp. rate & Non-zeros [\%]&$\max(\sigma^2)$ & $\text{mean}(\sigma^2)$ &$\text{Var}(\sigma^2)$\\ 
\hline  \hline 
0.005	& 10 & 4.3  & 27.1 & 12.1 & 0.0050 & 0.0050 & 0.000\\	%3 0.00500036 0.00500525 1.49193e-12
0.005  	& 100 & 3.9  & 24.8 & 13.1& 0.0050 & 0.0050 & 0.000\\%4 0.00500523 0.00508479 3.95693e-10
0.05	& 1000 &  1.8 & 60.7 & 4.3 &0.475 & 0.0711&0.010\\	%1 0.071163 0.475351 0.0103382
\hline
\end{tabular}
\end{center}
\label{table:gamma}
\end{table}

